What are the attackers doing now? Automating cyber threat intelligence extraction from text on pace with the changing threat landscape: A survey

Cybersecurity researchers have contributed to the automated extraction of CTI from textual sources, such as threat reports and online articles, where cyberattack strategies, procedures, and tools are described. The goal of this article is to aid cybersecurity researchers understand the current techniques used for cyberthreat intelligence extraction from text through a survey of relevant studies in the literature. We systematically collect "CTI extraction from text"-related studies from the literature and categorize the CTI extraction purposes. We propose a CTI extraction pipeline abstracted from these studies. We identify the data sources, techniques, and CTI sharing formats utilized in the context of the proposed pipeline. Our work finds ten types of extraction purposes, such as extraction indicators of compromise extraction, TTPs (tactics, techniques, procedures of attack), and cybersecurity keywords. We also identify seven types of textual sources for CTI extraction, and textual data obtained from hacker forums, threat reports, social media posts, and online news articles have been used by almost 90% of the studies. Natural language processing along with both supervised and unsupervised machine learning techniques such as named entity recognition, topic modelling, dependency parsing, supervised classification, and clustering are used for CTI extraction. We observe the technical challenges associated with these studies related to obtaining available clean, labelled data which could assure replication, validation, and further extension of the studies. As we find the studies focusing on CTI information extraction from text, we advocate for building upon the current CTI extraction work to help cybersecurity practitioners with proactive decision making such as threat prioritization, automated threat modelling to utilize knowledge from past cybersecurity incidents.

==> backup.tex <==
Li et. al define APT as ``a cyber attack launched by a group of sophisticated, determined, and coordinated attackers who systematically compromise the network of a specific target machine or entity for a prolonged period'' \cite{li2011evidence}. For example, one of the APT attack examples which is mentioned in \cite{alshamrani2019survey} is \textit{Carbanak}. These attacks are started in 2013 and continued to 2017 with the goal of stealing money from financial institutions. The attackers attack up to 100 financial institutions and total financial losses were as high as \$1 billion \cite{carbanak}.
    
A zero-day attack is a cyberattack that occurs on the same day a vulnerability is discovered. so, it is exploited before a fix becomes available to prevent it \cite{zerodayexploit}.

 

% \subsection{Advanced Persistent Threat (APT)}
% Li et. al define APT as ``a cyber attack launched by a group of sophisticated, determined, and coordinated attackers who systematically compromise the network of a specific target machine or entity for a prolonged period'' \cite{li2011evidence}. For example, one of the APT attack examples which is mentioned in \cite{alshamrani2019survey} is \textit{Carbanak}. These attacks are started in 2013 and continued to 2017 with the goal of stealing money from financial institutions. The attackers attack to up to 100 financial institution and total financial losses were as high as \$1 billion \cite{carbanak}.

% \subsection{Indicator of Compromise (IoC)}
% Indicators of Compromise (IoC) refers to the artifacts of operating systems, applications, programs, and networks which indicate compromise, intrusion, or breach of computing systems \cite{gragido2012understanding}. IoC can be categorized in to three categories \cite{tounsi2018survey}: 1) Network indicators, such as IP addresses, URLs, and domain names; 2) Host-based indicators, such as malware names, malicious file hashes, and registry keys; 3) Email indicators, such as source email addresses, attachments, and links.

% \begin{table}[]
%     \centering
%     \caption{IoC categories and examples}
%     \label{tab:iocs}
%     \begin{tabular}{L{4cm}L{2cm}r}
%          \toprule
%          \textbf{IoC category} & \textbf{Description} & \textbf{Example}\\ \midrule
%          Network indicators &   & \\ \midrule
%          Host-based indicators &  & \\ \midrule
%          Email indicators &  & \\ \midrule
%          \bottomrule
%     \end{tabular}
% \end{table}

% \subsection{CTI Sharing}\label{section:sharing}
% CTI sharing play a key role in surviving from current and future cyber attacks proactively \cite{wagner2019cyber}. Structured formats are defined for CTI description and sharing such as Structured Threat Information eXpression (STIX) \cite{stix}, Trusted Automated eXchange of Indicator Information (TAXII) \cite{taxii}, Open Threat Partner Exchange (OpenTPX) \cite{opentpx}, Malware Attribution Enumeration and Characterization (MAEC) \cite{maec}, Incident Object Description Exchange Format (IODEF) \cite{iodef}, Vocabulary for Event Recoding and Incident Sharing (VERIS) \cite{veris}, and OpenIoC \cite{openioc}.  
%\subsubsection{Structured Threat Information eXpression (STIX)}STIX is a structured language and serialization format for CTI sharing. STIX information is human and machine readable in JSON and contains domain and relation objects \cite{stix}.
%\subsubsection{Trusted Automated eXchange of Indicator Information (TAXII)}
%TAXII is an application protocol to share CTI over HTTPS \cite{taxii}.
%\subsubsection{Open Threat Partner Exchange (OpenTPX)}
%OpenTPX is an open source JSON-based format and tool for sharing machine-readable threat intelligence \cite{opentpx}.
%\subsubsection{Malware Attribution Enumeration and Characterization (MAEC)}
%MAEC is a standardized langauge for sharing structured information about malware \cite{maec}.
%\subsubsection{Incident Object Description Exchange Format (IODEF)}
%IODEF is a data representation framework for sharing computer security incidents' information in XML \cite{iodef}.
%\subsubsection{Vocabulary for Event Recoding and Incident Sharing (VERIS)}
%VERIS is a language to describe security incidents structured and repeatable \cite{veris}.

% \subsection{CTI Actionability}
% Wagner et.al \cite{wagner2019cyber} consider two definition of CTI actionability from Pawlinski et. al \cite{pawlinski2014actionable} and Ponemon Institute \cite{ponemon2014exchanging} to explain what is CTI actionability. CTI is actionable if it fulfills following criteria: relevance, timeliness, accuracy, completeness, ingestibility, priority, implementation, trustworthiness of the source, relevance to the industry, clear guidance to resolve the threat, and sufficient context. 

% \subsubsection{Timeliness of sharing CTI}
% \subsubsection{Trustworthiness of CTI sharing}
% \subsubsection{Stakeholder reputation}
% \subsubsection{Relevance of CTI}
% \subsubsection{Privacy \& anonymity}
% \subsubsection{Data interoperability}

% \subsection{Open Source Intelligence (OSINT)}
% OSINT is referred to a information which is legally and ethically is available in public resources \cite{steele1995importance} such as newspapers, magazines, social networking
% sites (e.g. twitter), and blogs. Cybersecurity OSINT sources which provide information related to security
% vulnerabilities, threats and attacks can be divided into two abstract groups \cite{mittal2016cybertwitter}: 1) formal sources such as NIST’s National Vulnerability Database (NVD), and 2) informal sources such as blogs, forums, and twitter. Information on these cybersecurity OSINT resources is published daily in large scale. Manual extraction of valuable information from these fast-changing resources is time-consuming and inefficient. So, automatically
% extracting relevant information from OSINT sources has received attention from the research community \cite{mittal2016cybertwitter}.

% With the increase of cyberattack incidence, the volume of available textual description of these attack from various sources has also increased. Security researchers and practitioners can avail these textual description to extract threat intelligence and gain insight on the attackers. In this section, we discuss the overall text mining pipeline for extracting threat intelligence from unstructured text found in the selected studies. First, we discuss the CTI mining purposes found in the studies. Then, we discuss the data sources from where cyberthreat related information can be gathered followed by approaches for data annotation and pre-processing. After that, we discuss the text mining techniques followed by various application scenario explored by the researchers. 

% and ~\cite{williams2018incremental}, SVM \cite{cortes1995support} and recurrent neural network \cite{medsker2001recurrent} are used respectively.

% The actionability of CTI helps organizations to improve their defense mechanisms. Wagner et.al \cite{wagner2019cyber} consider two definitions of CTI actionability from Pawlinski et. al \cite{pawlinski2014actionable} and Ponemon Institute \cite{ponemon2014exchanging} to explain CTI actionability. CTI is actionable if it fulfills the following criteria: relevance, timeliness, accuracy, completeness, ingestibility, priority, implementation, trustworthiness of the source, relevance to the industry, clear guidance to resolve the threat, and sufficient context. 

% Sharing CTI has the potential to aid in proactively protecting from current and future cyberattacks \cite{wagner2019cyber}. Structured formats have been defined for CTI description and sharing, such as Structured Threat Information eXpression (STIX) \cite{stix}, Trusted Automated eXchange of Indicator Information (TAXII) \cite{taxii}, Open Threat Partner Exchange (OpenTPX) \cite{opentpx}, Malware Attribution Enumeration and Characterization (MAEC) \cite{maec}, Incident Object Description Exchange Format (IODEF) \cite{iodef}, Vocabulary for Event Recoding and Incident Sharing (VERIS) \cite{veris}, and OpenIoC \cite{openioc}. The most used sharing format is STIX which is human and machine readable in JSON and contains domain and relation objects \cite{stix}.

\subsection{CTI Extraction}
\label{cti-extraction}
According to the definitions of CTI presented in Section~\ref{cti-def}, CTI is a set of information that can be used to prevent and defend against cyberattacks. Hence, any kind of device-to-device communication data, network/system/application logs, stack-traces, malware signatures, news/reports/articles of attacks in the context of a cybersecurity-related incident are sources for CTI. However, the usefulness of collected CTI depends on the accuracy, relevance, and soundness of the extracted information. CTI extraction process from these aforementioned sources was first orchestrated by human operators but that proved to be error-prone and inefficient, paving the opportunity for automatic extraction of CTI-related information~\cite{zhao2020timiner}. As the number and means of cyberattacks have grown with time, the textual descriptions and analysis of cyberthreat-related documents, reports, online articles, and online community interactions have grown as well. These textual documents of cyberthreat related activities are a valuable source for collecting CTI related information. Automatically extracting CTI information from these textual sources has already been explored by the cybersecurity researchers and in this survey, we focus on their CTI extraction goals, sources, approaches, and how the information is put to applications.  

Threat related activities such as attackers' TTPs; tools used by the attackers such as malicious scripts; details of malware, zero day bugs, vulnerabilities, exploits; cyberthreat related news and events related information can be found on these textual representation. Cybersecurity vendors and practitioners produce these information through monitoring threat activities, and collecting raw data from firewall, network logs, past security incidents. These data can help researchers and practitioners to gain insight on the threat landscape and form strategies to secure the systems from cyberattacks. 

The following example shows an excerpt of a threat report published by Palo Alto~\cite{paloalto-threat-report-example} covering possible threats on oil and gas organization. The excerpt demonstrates how an attacker can install malicious executable modules to illegally log into remote networks with stolen credentials. Through text mining, these attack techniques and tactics can be extracted into structured formats to further facilitate threat prevention mechanism. 

\begin{tcolorbox}
The sample submitted to VirusTotal is a Disttrack dropper, which is responsible for installing a communications and wiper module to the system. The dropper is also responsible for spreading to other systems on the same local network, which it accomplishes by attempting to log into other systems on the network remotely using previously stolen usernames and passwords.
\end{tcolorbox}

\subsubsection{Cyberthreat related dataset generation}
Threat intelligence information represented in structured format (i.e. STIX, graph databases) facilitates building cyberthreat knowledge base, sharing and collaboration among security researchers and practitioners. In the selected studies, researchers converted the extracted CTI relevant information into datasets of structured formats. In the selected studies, the types of CTI information stored into structured format are given below.

\begin{itemize}[leftmargin=3mm]

    \item \textbf{Malware information:} In ~\cite{piplai2020creating}, the authors extracted the malware related entities from text using NER, identified the relationship of the extracted entities using Unified cybersecurity ontology and then stored the entities with their relationship in a graph database. 
    
    \item \textbf{Vulnerability information:} In ~\cite{joshi2013extracting}, the authors extracted the vulnerabilities related entities from text using NER, identified the relationship of the extracted entities using Unified cybersecurity ontology and then stored the entities with their relationship in a graph database. In ~\cite{mulwad2011extracting}, the authors extracted the vulnerability relevant information by querying Wikipedia and Wikitology concepts and then stored the entities and their relationship in a graph database based on IDS ontology.
    
    \item \textbf{Cyberthreat events:} In one study, researchers also constructed dataset for cyberthreat related event detection. In~\cite{trong2020introducing}, the authors manually annotated articles from thehackernews website with 30 types of cybersecurity related events and then used supervised learners to validate their labelling on the dataset.
\end{itemize}

Over the last several years, security researchers have applied automated techniques for gathering threat intelligence to thwart cyberattacks. From the four sub-domain of CTI mentioned in Section~\ref{cti-def}, tactical threat intelligence can be extracted from textual documents regarding what attackers are currently doing and what can be the best practices to deter them~\cite{tounsi2018survey}. Moreover, technical threat intelligence information such as low-level information of malware signatures, malicious IP addresses and URLs are valuable for preparing and defending the organization from cyberattacks. Hence, researchers have deployed automated techniques to extract CTI information in different levels of abstractions. For example, many studies focused on only classifying the cyberthreat related posts in social media~\cite{shin2020new, deliu2018collecting}. On the other hand, many studies focused on identifying low-level attack tactics, techniques, and procedures~\cite{husari2017ttpdrill, husari2018using}. 
